Better Coherence, Better Height: Fusing Physical Models and Deep Learning for Forest Height Estimation from Interferometric SAR Data

Estimating forest height from Synthetic Aperture Radar (SAR) images often relies on traditional physical models, which, while interpretable and data-efficient, can struggle with generalization. In contrast, Deep Learning (DL) approaches lack physical insight. To address this, we propose CoHNet - an end-to-end framework that combines the best of both worlds: DL optimized with physics-informed constraints. We leverage a pre-trained neural surrogate model to enforce physical plausibility through a unique training loss. Our experiments show that this approach not only improves forest height estimation accuracy but also produces meaningful features that enhance the reliability of predictions.

==> sec/4_experiments_bkp.tex <==
\section{Experiments}

% Start with data description. Show examples. Show and discuss main results. Start with forest height, then with optimized coherence. Then show parameter studies.
\textbf{Dataset}: During training, ground truth height from the AfriSAR campaign is used. AfriSAR campaign is a NASA-ESA joint campaign that collected ground airborne SAR and airborne LiDAR data for the development and evaluation of forest structures and biomass retrieval algorithm, and NASA, GEDI, and BIOMASS sensor calibration \cite{fatoyinbo2021nasa}. Study area for the AfriSAR campaign was Gabon as it is is densely forested country with rich structural and functional biodiversity. The five imaged site as part of the campaign were Mondah forest, Lope National Park, Mabounie, Rabi, and Pongara National Park. For this study, the already gridded  forest characterizaion products derived from full-waveform lida data acquired by NASA's airborne Land, Vegetation and Ice Sensor (LVIS) instrument is used. It contains geolocated canopy cover a spatial resolution of 25m  that is readily processed to Level 3 (l3a1) product RH98 which is the mean relative height at which 98\% waveform energy occurs. 

The corresponding SAR accquisitons for this region was obtained from Tandem-X (DLR) satellite mission. In 2016, Tandem-X was operated on the coinciding regions of AfriSAR region for further scientific experiments with bistatic modes of operation. The SAR images used in this study is CoSSC (Co-registered Single Look Slant Range Complex) product \cite{fritz2012interferometric} and derived features. Bistatic sensors such as TanDEM-X consist of two satellites flying in a close formation separated by a spatial baseline acquiring SAR data simultaneously from the same area. The two acquired SAR images are focused and spatially aligned before being used for further processing.
The InSAR-derived feature complex coherence is the pixel-wise product of the SLCs (with one of them complex conjugated) and normalized with both their magnitudes.  It is a cross-correlation factor providing insights into the coherence [absolute value range 0 - 1] or similarity of radar scattering properties between two acquisitions. High coherence values are consistent with stable scatterers (eg. building) present in the scene and low coherence values are indicative of a change in scatterers due to various decorrelation factors and contain valuable information about volumetric scattering due to vegetation. \\
\textbf{Evaluation Metrics}: In order to test our model we use Root Mean Squared Error (RMSE) and coefficient of determination ($R^2$) which are defined in Equation 1 and Equation 2. Where $y_i$ is the ground truth height measurements and $\hat{y}_i$ is the predicted height. 
\begin{equation}
\text{RMSE} = \sqrt{\frac{1}{n} \sum_{i=1}^{n} (y_i - \hat{y}_i)^2}
\end{equation}

\begin{equation}
R^2 = 1 - \frac{\sum_{i=1}^{n} (y_i - \hat{y}_i)^2}{\sum_{i=1}^{n} (y_i - \bar{y})^2}
\end{equation}
\textbf{Implementation}: Patch based method is utilized for the training. The images are divided into patched of size 64 x 64 with a stride of 32. The different architectures are used in different experimental setups are explained in the following section of the paper. Training was performed for 100 epochs with a batch size of 8 and a learning rate varying between $10^{-4}$ and  $10^{-3}$. 

\subsection{Comparison with State of Art (SOTAs)}
\textbf{Direct-Method Scenario}: In order to analyze the performance of the established End-to-End model we set up baseline model with a state of the art U-net architecture as in \cite{mahesh2024forest} for comparisons. A direct input - output mapping is learned between the input coherence parameter and the ground truth LVIS forest heights. We consider four dataset regions from the AfriSAR compaign i.e. Mabounie, Rabi, Pongara, Lope. For each of the region, the training and validation splits are created image wise where a single image is for validation and remaining images are used for training purposes. The number of training images used for Mabounie is 5 nos, Rabi is 4 nos, Pongara is 2 nos and Lope is 1 nos while each region has 1 nos of validation image. The selection of train and test was performed in away that the training and the validation sample contains similar data distributions. The mean height distribution for all the datsets is in between 30 and 40 m. In supplementary material we further demonstrate with K-fold validation technique the statistical analysis of the independent datasets. In addition to the four datasets resulting from four region, a combined dataset is created that consists of all the four regions with total of 12 nos of training images and 4 nos of validation images, which is the sum of the original validation splits from each of the 4 regions. \\
In training phase five independent models are trained which includes a model for each of the four regions and a combined model over all the four regions together. The model weights are randomly initialized. Impact of random weight initialization on the RMSE performance has been evaluated in studies on  dataset regions \cite{carcereri2023deep} \cite{mahesh2024forest} and the overall variability was found to be in few decimeters. This indicates that the random initialization in this task for this data does not cause learning unstability and  provides consistent model performance on different runs. Therefore single experimentation runs are conducted in this study.\\ 
Evaluation is performed only the pixels where the ground truth target are available. RMSE performance of the resulting models is given by the diagonal of the confusion matrix shown in Figure \ref{fig:conf_matrix_direct_model}. The y-axis corresponds to the distinct models trained independently on different dataset regions i.e Mabounie, Rabi, Pongara, Lope and Gabon (combined model). The X-axis corresponds to the dataset regions on which the the different trained models are inferenced to analyze its generalization or spatial transfer capabilities. The best performing model on each of the dataset region is observed to be the combined Gabon model. RMSE error of this trained model varies between 5.2 to 6.71 m on different dataset regions. Models trained and evaluated on the same dataset regions have an 4.2 \% to 12.1\%  increased RMSE error against the combined Gabon model evaluated on these individual regions. Performance of all the models drops when evaluated on Lope region with the exception of Lope model which indicates a data distribution shift in this region where the trained direct models learn "shortcuts" based on the region-specific patterns that don't exist in other regions, therefore doesn't generalize well. Furthermore Rabi model's performance struggles on other regions with highest errors of 15.7 m on Lope showing the importance of including the different data characteristics in the training data as in combined Gabon model which reduces the error to 6.08 m when evaluated on all the regions together. The coefficient of determination ($R^2$) for all the models are provided in the Supplementary Material. 

\begin{figure}
    \centering
    \includegraphics[width= 1\linewidth]{Images/Confusion_Matrix_Direct_Model.pdf}
    \caption{Performance of Direct-Method Scenario on all Dataset Region with Spatial Transfer Analysis.}
    \label{fig:conf_matrix_direct_model}
\end{figure}

\noindent \textbf{Pre-trained Neural Surrogate Physical Model}
A physics engine can be used to enforce the physics plausibility but these are not differentiable, rely on assumptions, and are difficult to integrate into the learning framework. Therefore for the training of the End-To-End model in our approach, we pre-train a surrogate model to leverage  physics principles, particularly Random Volume over Ground Model (RVOG), to capture the relationship between the radar backscatter and forest height. The results of the pretraining are given in Figure \ref{fig:conf_matrix_physics_model}. Overall, a good agreement is obtained between the prediction and the physical model simulated forest height for all the regions, including the combined Gabon model. For models trained on self-regions, the error varied between 0.955 to 3.52 m RMSE and the combined Gabon model trained and evaluated on other regions had an error varying between 0.973 to 2.18 m RMSE. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Images/Confusion_Matrix_Physics_Surrogate_Model.pdf}
    \caption{Performance of Pre-trained Neural Surrogate Physical Model with Spatial Transfer Analysis}
    \label{fig:conf_matrix_physics_model}
\end{figure}

\noindent\textbf{End-to-End Model Training Evaluation}
We evaluate the performance of our end-to-end model framework trained with their self-region neural surrogate model. We first look at the forest height estimates from this model using the optimized coherence parameter produced by the first network. Figure \ref{fig:conf_matrix_End_to_End_Model} shows the RMSE performance of the End-to-End model. The best-performing model on each of the dataset regions is observed to be the combined Gabon model. RMSE error of this trained model varies between 5.97 to 8.62 m. Models trained and evaluated on the same dataset regions have a 4.6 \%  to 9.5\% against the combined Gabon model. When the end-to-end model is compared against the direct model most of the models have slightly higher errors than the direct model ranging from 0.71 to 2.01 m. A performance increase is noticed for the Rabi region where the end-to-end model performs better than the direct model with lower errors ranging from - 1.22 to - 6.59 m except for the self-trained region where the error is 0.71 m
Figure \ref{fig:conf_matrix_ETE_vs_Direct} shows the difference error against the direct model. Figure \ref{fig:feature_maps_all_regions} shows the qualitative results obtained with end-to-end training for the regions with the Gabon model with maps generated for coherence-related parameters such as volumetric decorrelation, optimized coherence, and height-related parameters such as  physical model forest height, target LVIS RH98 height, end-to-end model predicted height and the error for predicted height vs. target height. 



\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Images/Confusion_Matrix_ETE_Model.pdf}
    \caption{Performance of End-to-End trained Model with Spatial Transfer Analysis}
    \label{fig:conf_matrix_End_to_End_Model}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width= 1\linewidth]{Images/Confusion_Matrix_ETE_vs_Direct_Model.pdf}
    \caption{Performance Error Comparison of End-to-End Model against the Direct Model}
    \label{fig:conf_matrix_ETE_vs_Direct}
\end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.45\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Images/Vol_decorrelation.png}
%         \caption{Volume Decorrelation}
%         \label{fig:vol_decor}
%     \end{subfigure}%
%     \hspace{0.05\linewidth}
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Images/optimized_coherence.png}
%         \caption{Optimized Coherence}
%         \label{fig:pred}
%     \end{subfigure}%
%     \\
%     \begin{subfigure}[b]{0.45\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Images/PM_Height.png}
%         \caption{Physical Model Height}
%         \label{fig:pred}
%     \end{subfigure}%
%     \hspace{0.05\linewidth}
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Images/LVIS_RH98.png}
%         \caption{Target Height}
%         \label{fig:target}
%     \end{subfigure}%
%     \\
%     \begin{subfigure}[b]{0.45\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Images/Pred_Height.png}
%         \caption{Predicted Height}
%         \label{fig:pred}
%     \end{subfigure}%
%     \hspace{0.05\linewidth}
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Images/Error.png}
%         \caption{Error (Pred. - Target)}
%         \label{fig:pred}
%     \end{subfigure}
%     \caption{Qualitative results of forest height and optimized parameter with end-to-end training.}
%     \label{fig:feature maps}
% \end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{Images/Feature_Maps.png}
    \caption{Qualitative results for end-end-model trained Gabon model over the four regions: Mabounie, Rabi, Pongara, and op..Predictions are masked with forest and nonforest map (white regions)}
    \label{fig:feature_maps_all_regions}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{Images/Coherence_Maps.png}
    \caption{Qualitative comparison of different types of Coherence features in the end-to-end framework such as input coherence, volumetric decorrelation, optimized parameter, and the difference between the optimized parameter and the volumetric decorrrlation}
    \label{fig:cohernece maps}
\end{figure*}

\noindent \textbf{Advantages over Physics based Methods}
End-to-End model surpasses the existing simple physical models such as Random over ground Model (RVOG) without relying on the physics models for estimation. For instance although our model uses training data from physical model it is not required for inference and can be applied to regions aswell. 


\subsection{Ablation Study}
We study the effectiveness of the end-to-end framework by replacing the neural surrogate model used for the training of the end-to-end model with the combined Gabon neural surrogate model which has been trained over all the regions to include data characteristics from all the regions. Figure \ref{fig:conf_matrix_End_to_End_Model_Gabon_PM} shows the RMSE performance of the End-to-End framework model using the Gabon Neural Surrogate Model while Figure \ref{fig:conf_matrix_ETE_Gabon_PM_vs_Direct} and Figure \ref{fig:conf_matrix_ETE_Gabon_PM_vs_ETE} shows the error difference of this model against the direct method and the End-to-End Model respectively. The end-to-end model with the Gabon neural surrogate model has an RMSE performance similar to that of the End-to-End model with a regional neural surrogate model. The reduction of error is evident for lope models where the generalization of the model improves when evaluated on the other regions. Using a better physical model indicates that there is a possibility to reduce the error even further. The achieved performance critically depends on the definition of the inversion model. An oversimplified inversion model with strict assumptions results in a compromised performance of the model and the ability to generalize further. A complex or more robust version of the RVoG model can help resolve this issue and improve the overall performance of the end-to-end model. 
% can we run experiments here by also using weighting the physical informed loss or by adding coherence loss term ?. Also performance loss by reducing the training images ?.  

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Images/Confusion_Matrix_ETE_Gabon_PM_Model.pdf}
    \caption{Performance of End-to-End trained Model with Spatial Transfer Analysis using the Gabon Neural Surrogate Model}
    \label{fig:conf_matrix_End_to_End_Model_Gabon_PM}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Images/Confusion_Matrix_ETE_Gabon_PM_Model_vs_Direct_Model.pdf}
    \caption{Performance Error Comparison of the End-to-End Model with Gabon Neural Surrogate Model against Direct Model (ETE Gabon PM  -Direct Model) }
    \label{fig:conf_matrix_ETE_Gabon_PM_vs_Direct}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Images/Confusion_Matrix_ETE_Gabon_PM_Model_vs_ETE.pdf}
    \caption{Performance Error Comparison of the End-to-End Model with Gabon Neural Surrogate Model against End-to-End Model (ETE Gabon PM - ETE Model) }
    \label{fig:conf_matrix_ETE_Gabon_PM_vs_ETE}
\end{figure}



\subsection{Evaluation of Optimized Parameter}
In preceding sections, we show that the End-To-End model generates more physically-consistent estimates and produce reasonable forest height. 
The improved output from the network can successfully improve downstream task such as the forest height estimation. We demonstrate this through the evaluation of the optimized parameter. We compare the optimized parameter generated by our network against the computed coherence and volumetric decorrelation. Specifically, we employ the pre-trained physical model deep learning approximator to invert forest height and evaluate the accuracy against the ground truth LVIS height measurements. Density scatter plot with respective marginal distribution  for the different coherence parameters utilized are shown in figure \ref{fig:scatter_plots}. It is observed that the End-to-End model generated optimized parameter yields the best performance with an RMSE error of 7.35 m and $R^2$ = 0.55. Particularly while using the first processing level parameter coherence yields an RMSE of 17.24m ($R^2$ = -1.5) and second processing level  volumetric decorrelation yields  RMSE of 16.26 m  ($R^2$ = -1.2). Note that by using the optimized parameter for height inversion we are able to cut the error againt the LVIS ground truth by 50\% and demonstrate the effectiveness of the approach to align with the ground truth all the while enforcing physics information.

\begin{figure*}[ht]
    \centering
    \begin{subfigure}{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/density_scatter_Coh_H_vs.TargetH_13(2).png}
        \caption{Coherence Input}
        \label{fig:Coherence Parameter}
    \end{subfigure}%
    \hspace{0.05\textwidth}
    \begin{subfigure}{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/density_scatter_Vol_Decor_H_vs.TargetH_13.png}
        \caption{Volumetric Decorrelation Input}
        \label{fig:image2}
    \end{subfigure}%
    \hspace{0.05\textwidth}
    \begin{subfigure}{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/density_scatter_PredH_vs.TargetH_13.png}
        \caption{Optimized Parameter Input}
        \label{fig:image3}
    \end{subfigure}
    \\
     \begin{subfigure}[b]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/density_scatter_Opt_parm_vs.Coh_13.png}
        \caption{Opt. Parameter vs. Coherence }
        \label{fig:pred}
    \end{subfigure}%
    \hspace{0.05\textwidth}
    \begin{subfigure}{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/density_scatter_Opt_parm_vs.Target_Vol_Decor_13.png}
        \caption{Opt. Parameter vs. Vol. Decorrlation}
        \label{fig:pred}
    \end{subfigure}
    \caption{Density scatter plots for height inversion via pre-trained physical model Deep Learning Approximator[a,b,c] and Optimized Parameter against Coherence and Volumetric Decorrlation [d, e].}
    \label{fig:scatter_plots}
\end{figure*}

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.45\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Images/density_scatter_Opt_parm_vs.Coh_13.png}
%         \caption{Opt. Parameter vs. Coherence }
%         \label{fig:pred}
%     \end{subfigure}%
%     \hspace{0.05\linewidth}
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Images/density_scatter_Opt_parm_vs.Target_Vol_Decor_13.png}
%         \caption{Opt. Parameter vs. Vol. Decorrlation}
%         \label{fig:pred}
%     \end{subfigure}
%     \caption{Desnity Scatter P
% lots for Optimized Parameter against Volumetric Decorrelation and Cohernece.}
%     \label{fig:opt_scatter}
% \end{figure}
